Clinically Relevant Latent Space Embedding of Cancer Histopathology Slides through Variational Autoencoder Based Image Compression

In this paper, we introduce a Variational Autoencoder (VAE) based training approach that can compress and decompress cancer pathology slides at a compression ratio of 1:512, which is better than the previously reported state of the art (SOTA) in the literature, while still maintaining accuracy in clinical validation tasks. The compression approach was tested on more common computer vision datasets such as CIFAR10, and we explore which image characteristics enable this compression ratio on cancer imaging data but not generic images. We generate and visualize embeddings from the compressed latent space and demonstrate how they are useful for clinical interpretation of data, and how in the future such latent embeddings can be used to accelerate search of clinical imaging data.

==> sections/results.tex <==
\section{Results}
\label{sec:results}
    
    Fig. \ref{fig:4}-a shows the impact of various compression ratios on VAE output images. At lower compression ratios, reconstructed images more closely resemble original input images. Importantly, we see a marked improvement in histologic features that are critical for interpretability such as refined cell-to-cell borders and sharper demarcation of cytoplasmic vs. nuclei compartments.
    
  

    Moreover, in Fig. \ref{fig:4}-b, we use UMAP to visualize the latent space vectors learned by our pipeline. The UMAP captures intra-tumor and across-tumor relationships, separating all four tissue types into distinct clusters. Interestingly, clusters of brain and colon cancers share overlapping boundaries whereas the breast cancer cluster is uniquely separated from the brain cancer cluster. Additionally, the UMAP identifies a distinct sub-cluster of brain tumor samples that does not overlap with any other cancer types. 

    
  
